A Convex Framework for Fair Regression

We introduce a flexible family of fairness regularizers for (linear and logistic) regression problems. These regularizers all enjoy convexity, permitting fast optimization, and they span the rang from notions of group fairness to strong individual fairness. By varying the weight on the fairness regularizer, we can compute the efficient frontier of the accuracy-fairness trade-off on any given dataset, and we measure the severity of this trade-off via a numerical quantity we call the Price of Fairness (PoF). The centerpiece of our results is an extensive comparative study of the PoF across six different datasets in which fairness is a primary consideration.

==> exp-comparison.tex <==
\subsection{Comparison with Existing Approaches}

\sj{how do we compare with other post-processing or in-processing
approaches defined previously? What are meaningful baseline?
For post-processing in classification~\cite{HardtPS16} is a good candidate.
For post-processing baseline in regression mixing with any constant vector
seems like a good candidate.}
